Price formation in financial markets: a game-theoretic perspective

We propose two novel frameworks to study the price formation of an asset negotiated in an order book. Specifically, we develop a game-theoretic model in many-person games and mean-field games, considering costs stemming from limited liquidity. We derive analytical formulas for the formed price in terms of the realized order flow. We also identify appropriate conditions that ensure the convergence of the price we find in the finite population game to that of its mean-field counterpart. We numerically assess our results with a large experiment using high-frequency data from ten stocks listed in the NASDAQ, a stock listed in B3 in Brazil, and a cryptocurrency listed in Binance.

==> ADF_tableOrderFlowImbalancewithmicroimpact <==
\begin{longtable}{llrl}
\caption{ADF statistics on $d-$fractional differenciated price series}\\
\toprule
     stocks &    $ADF$ &   $d$ & Correlation \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
      PETR4 & -7.55231 &  0.01 &    0.999955 \\
      VALE3 & -9.83917 &  0.04 &     0.98586 \\
      MGLU3 & -10.3368 &  0.03 &    0.997506 \\
      ITUB4 &  -8.4521 &  0.05 &    0.979125 \\
      BBDC4 & -13.0457 &  0.03 &    0.996615 \\
      VVAR3 &  -5.8886 &  0.06 &    0.990677 \\
      PETR3 & -9.81691 &  0.02 &    0.998482 \\
      BBAS3 & -5.45667 &  0.01 &    0.999911 \\
      ABEV3 & -20.7615 &  0.10 &    0.942916 \\
      JBSS3 & -6.58439 &  0.02 &    0.999307 \\
 Grand mean & -9.77342 &  0.04 &    0.989035 \\
\end{longtable}


==> Empirical.tex <==
\section{Empirical assessments I: the MFG setting} \label{sec:Empirical}

\subsection{The data} \label{subsec:data}

%[\textbf{WHERE OUR DATASETS COME FROM, WHAT DOES IT COMPREHENDS, HOW DID WE TREAT IT ETC.}]

The data we use in this work can be found at \href{http://sebastian.statistics.utoronto.ca/books/algo-and-hf-trading/data/}{http://sebastian.statistics.utoronto.ca/books/algo-and-hf-trading/data/}.  It is from November 2014 for the following tickers: AMZN, EBAY, FB, GOOG, INTC, MSFT, MU, PCAR, SMH, VOD. This data contains all trades and snapshots of the LOB for every 100ms of the trading day.  In Table \ref{tab:stocksData},  we display the mean and standard deviation in parenthesis for each stock,  of the midprice, spread, and average daily volume (ADV).

\begin{footnotesize}
\input{dataInfoTablePriceFormation}
\end{footnotesize}

\subsection{Results} \label{subsec:TI_MFG_Empirics}

% \todo{Come\c{c}ar falando da ref, venda trade imb}
Here, we assess the performance of the formula \eqref{eq:FormedPriceMFG} we obtained using the data we described in Section \ref{subsec:data}. From the market clearing condition \eqref{eq:MktClearingMFG}, we see that $\Lambda$ should be taken as the additive opposite of a measure of order flow. In the current experiments, we use the Trade Imbalance $\TI$ (see \cite{cont2014price}) as such a measure, which we now proceed to describe. Firstly, we divide the trading day $\left[0,T\right]$ in $12$ corresponding intervals $\left[0=T_0,T_1\right],\ldots,\left[T_{11},T_{12}=30\right].$ We assume parameters are constant in each of these time window of $30$ minutes $\left[T_i,T_{i+1}\right],$ further dividing such slice into smaller intervals $T_i = t_{i,0}<\ldots<t_{i,179} = T_{i+1}$ of constant length $t_{i,k+1}-t_{i,k}=10$ seconds. Secondly, we define the time series $\TI^i = \left\{ \TI^i_k \right\}_{k=0}^{179}$ on $\left[T_i,T_{i+1}\right]$ as
\begin{equation}\label{eq:tradeImbalance}
\TI^i_k = \sum_{n = N_{i,k} + 1}^{ N_{i,k+1} } \left\{ \mu^+_n - \mu^-_n \right\},  
\end{equation}
where $N_{i,k}$ denotes the number of events that have occurred on $\left[T_i,t_{i,k}\right],$ and $\mu^+_n$ (respectively, $\mu^-_n$) is the number (possibly zero) of buy (respectively, sell) market orders that are traded within $\left]t_{i,n-1},\,t_{i,n} \right],$ for each $n\geqslant 1.$ Then, we define the time series 

\begin{equation} \label{eq:TimeSeries_MFG}
    \begin{cases}   
        S^{i,0} := \left\{S^{i,0}_k := 1 \right\}_{k = 0}^{179},\, S^{i,1} := \left\{S^{i,1}_k := t_{i,k} \right\}_{k = 0}^{179},\\
        S^{i,2} := \left\{S^{i,2}_k := \int_{T_i}^{t_{i,k}} \Lambda(u)(t_{i,k}-u)\,du \right\}_{k = 0}^{179},\, S^{i,3} := \left\{S^{i,3}_k := \Lambda(t_{i,k}) \right\}_{k = 0}^{179}, 
    \end{cases}
\end{equation}
where we fix $\Lambda(t_{i,k}) = -\TI^i_{k}.$ In $S^{i,2}$ (see \eqref{eq:TimeSeries_MFG}) we use the Python method \texttt{scipy.integrate.cumtrapz} to compute the integral term. Thirdly, we undertake the subsequent regression over $\left[T_i,T_{i+1}\right]:$
\begin{equation} \label{eq:RegressionFormedPrice_MFG}
    \fp^i_k = a_{i,0} S^{i,0}_k + a_{i,1} S^{i,1}_k + a_{i,2} S^{i,2}_k + a_{i,3} S^{i,3}_k + \epsilon^i_k,
\end{equation}
where we denote the error term by $\epsilon^i_k$ and the observed price at time by $\fp^i_k$, both at time $t_{i,k}$. 


As a benchmark, we take a model inspired by \cite{kyle1985continuous}, viz.,
\begin{equation} \label{eq:RegressionTIBenchmark_MFG}
    \Delta \fp^i_k := \fp^i_k - \fp^i_{k-1} = b_{i,0} + b_{i,1} \TI^i_k + \widetilde{\epsilon}^i_k.
\end{equation}
Thus, in this benchmark, we simply assume that a price movement must correspond linearly to the market trade imbalance.

In Figure \ref{fig:ExampleOfTheFit}, we provide an example of the performance of our model with parameters estimated as we described above, i.e., via the regression \ref{eq:TimeSeries_MFG}, together with the benchmark model \ref{eq:RegressionTIBenchmark_MFG}. In Table \ref{MFG_FinitePopR2_oneStock}, we present the average over all windows of all trading days of November $2014$ for the INTC stock. Then, we present this average $R^2$ values corresponding to the other stocks of Table \ref{tab:stocksData}. We notice that the MFG model beats the model linear trade imbalance systematically, over all stocks we consider. We also showcase in Table \ref{tab:FormedPrice_TI} the average values over all windows of the parameters we estimate from the regression \eqref{eq:RegressionTIBenchmark_MFG}. We immediately interpret the parameter $a_0$ as the average initial price of the corresponding stock sampled at the beggining of each window. The remaining parameters are more intrically related to the fundamental ones of our model, but we can recover the latter by matching relations \eqref{eq:FormedPriceMFG} and \eqref{eq:RegressionFormedPrice_MFG}.

\begin{figure}[h]
\includegraphics[width=\textwidth]{INTC_formedPriceTI}
\caption{
We use the Trade Imbalance, $\TI$ (see \cite{cont2014price}), as a measure of order flow (see \eqref{eq:tradeImbalance}) and the MFG model coefficients of the formed price equation: 
$
    \fp^i_k = a_{i,0} S^{i,0}_k + a_{i,1} S^{i,1}_k + a_{i,2} S^{i,2}_k + a_{i,3} S^{i,3}_k + \epsilon^i_k,
$
where we denote the error term by $\epsilon^i_k$ and the observed price at time by $\fp^i_k$, both at time $t_{i,k}$.  Such regression is performed in time intervals of $30$ minutes $\left[T_i,T_{i+1}\right],$ where model parameters are kept constant.  Moreover, we divide each window of 30 minutes into smaller intervals $T_i = t_{i,0}<\ldots<t_{i,179} = T_{i+1}$ of constant length $t_{i,k+1}-t_{i,k}=10$ seconds.  This regression corresponds to the MFG model in Theorem \ref{thm:MainTheorem}. As a benchmark, we take a model inspired by \cite{kyle1985continuous}, viz.,
$
    \Delta \fp^i_k := \fp^i_k - \fp^i_{k-1} = b_{i,0} + b_{i,1} \TI^i_k + \widetilde{\epsilon}^i_k.
$
This benchmark was also considered in \cite{cont2014price}. }
\label{fig:ExampleOfTheFit}
\end{figure}



==> Empirical2.tex <==
\section{Empirical assessments II: the finite population setting} \label{sec:Empirics2_FinPop}

\subsection{Proceeding with the trade imbalance metric}

Here, we will employ the notations we fixed in Subsection \ref{subsec:TI_MFG_Empirics} with the process $\left\{\Lambda^N_t\right\}_t$ here playing the role that the continuous function $\Lambda$ did there. Under the assumptions of Corollary \ref{cor:ParticularCase1}, we let us define the term 
$$
I_{\text{micro}}(t) := \int_0^t \xi^N_u\left(\Lambda_u^N\right)\Lambda_u^N\,du.
$$
We notice that $I_{\text{micro}}$ figures in the price formation formula \eqref{eq:ParticularCase1} for the finite population game. We call it $I_{\text{micro}}$ since it appears due to the microscopic impact suffered by an individual trader as a market friction. If we assume, in particular, that this impact $\xi^N_u \equiv \xi^N$ is constant, then
$$
I_{\text{micro}}(t) = \xi^N \int_0^t \Lambda_u^N\,du.
$$
In the case of a decentralized game, it is reasonable to expect that $\xi^N = O(1/N),$ as we previously discussed \comm{(refer to a remark}). However, if there is some persistence in the impact of some ``special'' traders, as in a case when there is a hierarchy among the population, cf. \cite[Section 5]{evangelista2020finite}, we could expect that such a term would play a relevant role in the price formation process.

Inspired by this discussion, we assess the performance of the regressions \eqref{eq:RegressionFormedPrice_MFG} (over the time slices $[T_i,T_{i+1}]$) with one additional explanatory variable. Namely, we consider the time series
$$
S^{i,4} := \left\{S^{i,4}_k := \int_{T_i}^{t_{i,k}} \Lambda_u^N \,du \right\}_{k=0}^{179},
$$
for each window $\left[T_{i},T_{i+1}\right].$ In this way, the regressions of which we investigate the properties in the current section is
%\begin{equation} \label{eq:RegressionFinPop}
%    \fp^i = \beta_0^i S^{i,0} + \beta_1^i S^{i,1} + \beta_2^i S^{i,2} + \beta_3^i S^{i,3} + \beta_4^i S^{i,4} + \eta^i,
%\end{equation}
\begin{equation} \label{eq:RegressionFinPop}
    \fp_k^i = a_{i,0} S_k^{i,0} + a_{i,1} S_k^{i,1} + a_{i,2} S_k^{i,2} + a_{i,3} S_k^{i,3} + a_{i,0} S_k^{i,4} + \eta_k^i,
\end{equation}
where we denote the error term by $\eta^i_k$ and the observed price at time by $\fp^i_k$, both at time $t_{i,k}$. We first consider,  as in Section \ref{subsec:TI_MFG_Empirics}, that $\Lambda^N$ is given by the trade imbalance. 

We showcase in Figure \ref{fig:FormedPriceTI_finPop} the outcome of estimating the regression parameters according to \ref{eq:RegressionFinPop}, as compared to the trade imbalance linear model --- the same benchmark as Section \ref{subsec:TI_MFG_Empirics}. As in Section \ref{sec:Empirical}, we present in Table \ref{MFG_FinitePopR2_allStock} the average $R^2$ for the finite population model with the trade imbalance metric. We observe that the extra explanatory variable of the finite population game brings relevant information to the problem. Indeed, this novel model not only beats the benchmark considerably, buy it also improves the MFG model for all assets. The significance of the novel explanatory variable is an indication that there might be a persistent effect of certain players in the market.

\begin{figure}[h]
\includegraphics[width=\textwidth]{INTC_formedPriceTI_micro}
\caption{We use the Trade Imbalance, $\TI$ (see \cite{cont2014price}), as a measure of order flow (see \eqref{eq:tradeImbalance}) and compute the finite population game model coefficients of the formed price equation: 
$
    \fp^i_k = a_{i,0} S^{i,0}_k + a_{i,1} S^{i,1}_k + a_{i,2} S^{i,2}_k + a_{i,3} S^{i,3}_k +a_{i,4} S^{i,4}_k \eta^i_k,
$
where we denote the error term by $\eta^i_k$ and the observed price at time by $\fp^i_k$, both at time $t_{i,k}$.  Such regression is performed in time intervals of $30$ minutes $\left[T_i,T_{i+1}\right],$ where model parameters are kept constant.  Moreover, we divide each window of 30 minutes into smaller intervals $T_i = t_{i,0}<\ldots<t_{i,179} = T_{i+1}$ of constant length $t_{i,k+1}-t_{i,k}=10$ seconds. This regression corresponds to the finite population price model in Corollary \ref{cor:ParticularCase1}.  As a benchmark, we take a model inspired by \cite{kyle1985continuous}, viz.,
$\Delta \fp^i_k := \fp^i_k - \fp^i_{k-1} = b_{i,0} + b_{i,1} \TI^i_k + \widetilde{\epsilon}^i_k.$
This benchmark was also considered in \cite{cont2014price}.}
\label{fig:FormedPriceTI_finPop}
\end{figure}



\subsection{Taking queue sizes into account}

Henceforth, we will utilize a metric called Order Flow Imbalance (OFI), introduced in \cite[Subsection 2.1]{cont2014price}. The goal in using this is to take information from the LOB first queues into account. We proceed to provide the definition of $OFI$, referring to their paper for an in-depth discussion on its design. Maintaining the notations of Section \ref{subsec:TI_MFG_Empirics}, let us represent by $\fp^b_n$ and $q^b_n$ (respectively, $\fp^a_n$ and $q^a_n$) the bid (respectively, ask) price and volume (at-the-touch), respectively, resulting from the $n-$th set of events (i.e., those occurring within the window $\left]t_{i,n-1},\,t_{i,n}\right]$). We form the quantity
\begin{equation}\label{eq:enDef}
e_n := I_{\left\{ \fp^b_n \geqslant \fp^b_{n-1} \right\}}q^b_n -  I_{\left\{ \fp^b_n \leqslant \fp^b_{n-1} \right\}}q^b_{n-1} - I_{\left\{ \fp^a_n \leqslant \fp^a_{n-1} \right\}}q^a_n + I_{\left\{ \fp^a_n \geqslant \fp^a_{n-1} \right\}}q^a_{n-1},
\end{equation}
and we define
\begin{equation}\label{eq:OFIDef}
\OFI_k := \sum_{n = N_{i,k} + 1}^{N_{i,k+1}} e_n.
\end{equation}
The benchmark we consider to compare our results for this metric is then
$$
\Delta \fp_k^i = c_{i,0} + c_{i,1} \OFI_k^i + \overline{\epsilon}^i_k,
$$
where the regression is performed over the slice $\left[T_i,T_{i+1}\right]$,.
% \comm{which was studied in \cite{cont2014price}.}

The counterpart of \ref{fig:FormedPriceTI_finPop}, but with $\Lambda^N = -\OFI,$ is what we showcase in Figure \ref{fig:FormedPriceOFI_finPop}. This plot seems to indicate that using this metric does lead to better results than the trade imbalance one.

From the results of Tables \ref{MFG_FinitePopR2_oneStock} and \ref{MFG_FinitePopR2_allStock}, we notice that using the order flow imbalance metric leads to substantial improvement of the performance of the current model. Moreover, the model we derived also outperforms the benchmark. This highlights the importance of the memory term in the price formation process. However, the memory term does not seem to be the key of the performance boost relative to the pure linear in the OFI metric. Indeed, from Tables \ref{MFG_FinitePopR2_oneStock} and \ref{MFG_FinitePopR2_allStock}, we see that when we employ $\Lambda = \OFI,$ the average $R^2 $ of the the MFG model is worse overall. Thus, the most valuable term from the perspective of the OFI metric seems to be the last explanatory variable we introduced, in the form of the time series $S^4.$

\begin{figure}[h]
\includegraphics[width=\textwidth]{INTC_formedPriceOFI_micro}
\caption{We use the Oder Flow Imbalance, $\OFI$ (see \cite{cont2014price}), as a measure of order flow (see 
\eqref{eq:OFIDef}) and compute the finite population game model coefficients of the formed price equation: 
$
       \fp_k^i = a_{i,0} S_k^{i,0} + a_{i,1} S_k^{i,1} + a_{i,2} S_k^{i,2} + a_{i,3} S_k^{i,3} + a_{i,0} S_k^{i,4} + \eta_k^i,
$
where we denote the error term by $\eta^i_k$ and the observed price at time by $\fp^i_k$, both at time $t_{i,k}$.  Such regression is performed in time intervals of $30$ minutes $\left[T_i,T_{i+1}\right],$ where model parameters are kept constant.  Moreover, we divide each window of 30 minutes into smaller intervals $T_i = t_{i,0}<\ldots<t_{i,179} = T_{i+1}$ of constant length $t_{i,k+1}-t_{i,k}=10$ seconds.  This regression corresponds to the finite population game price model in Corollary \ref{cor:ParticularCase1}.  As a benchmark, we take the model introduced in \cite{cont2014price}, viz. , $\Delta \fp_k^i = c_{i,0} + c_{i,1} \OFI_k^i + \overline{\epsilon}^i_k$, where $\OFI$ and $e_n$ are given in \eqref{eq:OFIDef} and \eqref{eq:enDef} respectively.}
\label{fig:FormedPriceOFI_finPop}
\end{figure}

==> OFI_latex-table <==
\begin{longtable}{llllllllll}
\caption{Results for method ${OFI}$}\\
\toprule
      Stock &           $a_0$ &          $a_1$ &          $a_2$ &        $a_3$ &    $adf-resid$ &   $R^2_{OFI}$ &     $\alpha$ &      $\beta$ & $R^2_{bench}$ \\
\midrule
\endhead
\midrule
\multicolumn{10}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
         MU &      33.3967749 &      0.0633803 &      0.0006398 &       -8e-07 &     -2.7102019 &     0.5080833 &    -4.06e-05 &      1.6e-06 &     0.6348812 \\
            &     (0.8468794) &    (0.5352262) &    (0.0039691) &      (4e-07) &    (0.8779943) &   (0.2782342) &  (0.0002898) &      (5e-07) &   (0.1116312) \\
            &                 &                &                &              &                &               &              &              &               \\
         FB &      74.6863162 &     -0.1556568 &      0.0015774 &     -1.5e-06 &     -2.6450052 &     0.5499002 &    0.0001599 &      2.8e-06 &      0.646802 \\
            &     (0.9171862) &    (1.1302096) &    (0.0064471) &      (9e-07) &    (0.7881093) &   (0.2676806) &  (0.0009176) &      (1e-06) &   (0.1213636) \\
            &                 &                &                &              &                &               &              &              &               \\
       PCAR &      66.5653921 &     -0.0294768 &     -0.0044199 &     -6.3e-06 &     -2.6737082 &     0.5227527 &    -7.22e-05 &     1.15e-05 &     0.5943707 \\
            &     (0.6622394) &    (0.5652952) &    (0.0299058) &    (3.8e-06) &    (0.8936489) &    (0.276842) &  (0.0004809) &    (3.3e-06) &   (0.0919139) \\
            &                 &                &                &              &                &               &              &              &               \\
       AMZN &     317.2368614 &     -0.6234138 &      -0.005805 &    -3.45e-05 &     -2.6407034 &     0.5752787 &    0.0018582 &     6.83e-05 &      0.497083 \\
            &    (14.3359568) &    (4.2419751) &    (0.2407367) &   (2.49e-05) &    (0.8677074) &   (0.2578789) &  (0.0046468) &   (1.88e-05) &   (0.1019693) \\
            &                 &                &                &              &                &               &              &              &               \\
       EBAY &      54.1112839 &      0.0322441 &        6.2e-06 &     -1.5e-06 &     -2.7019206 &     0.5161722 &     4.68e-05 &        3e-06 &     0.6237341 \\
            &     (0.6804996) &    (0.4207827) &    (0.0079721) &      (9e-07) &    (0.9061468) &    (0.276937) &    (0.00035) &      (8e-07) &   (0.1201012) \\
            &                 &                &                &              &                &               &              &              &               \\
        SMH &      52.5152296 &      0.0492334 &     -0.0002052 &       -6e-07 &      -2.728325 &     0.5273391 &     -9.6e-06 &      1.1e-06 &     0.5366392 \\
            &     (1.0414812) &    (0.3983075) &    (0.0028926) &      (4e-07) &    (0.9110345) &   (0.2483619) &  (0.0003551) &      (3e-07) &    (0.112495) \\
            &                 &                &                &              &                &               &              &              &               \\
       INTC &      34.4930448 &       0.027989 &      0.0001221 &       -3e-07 &     -2.7783947 &     0.5356633 &     1.25e-05 &        8e-07 &     0.6298803 \\
            &     (1.1371134) &    (0.4241576) &    (0.0017873) &      (2e-07) &    (0.8585606) &   (0.2681156) &  (0.0002294) &      (2e-07) &     (0.09795) \\
            &                 &                &                &              &                &               &              &              &               \\
        VOD &      34.5712094 &     -0.0016934 &      -3.48e-05 &       -5e-07 &     -2.6613811 &     0.5577175 &     1.14e-05 &      1.2e-06 &     0.5950157 \\
            &     (1.2337536) &    (0.2765899) &     (0.003385) &      (4e-07) &    (0.9079183) &   (0.2822306) &  (0.0001424) &      (4e-07) &   (0.1315352) \\
            &                 &                &                &              &                &               &              &              &               \\
       GOOG &     542.8337984 &     -0.0967683 &     -0.0168942 &    -4.72e-05 &     -2.6882949 &     0.5928375 &    0.0006758 &     9.34e-05 &     0.4950987 \\
            &     (6.1530034) &     (4.533289) &    (0.3071193) &    (3.9e-05) &    (0.8744376) &   (0.2629105) &  (0.0055439) &   (2.64e-05) &   (0.0956888) \\
            &                 &                &                &              &                &               &              &              &               \\
       MSFT &      48.3945697 &      0.0601091 &      -7.33e-05 &       -4e-07 &     -2.7098915 &     0.5251484 &    -4.43e-05 &        8e-07 &     0.6882648 \\
            &     (0.7236829) &     (0.469177) &    (0.0020162) &      (2e-07) &    (0.9070437) &   (0.2760493) &  (0.0002614) &      (2e-07) &   (0.0949067) \\
            &                 &                &                &              &                &               &              &              &               \\
 Grand mean &  104.0421379498 &  -0.0900679855 &  -0.0016339368 &  -7.6827e-06 &  -2.6876183284 &  0.5363502751 &  0.000274322 &  1.50546e-05 &  0.5966037586 \\
\end{longtable}


==> OFI_latex-table-no-r2 <==
\begin{table}
\centering
\caption{Results for method ${OFI}$}
\begin{tabular}{llllllll}
\toprule
Stock &         $a_0$ &        $a_1$ &        $a_2$ &       $a_3$ &  $adf-resid$ &     $\alpha$ &     $\beta$ \\
\midrule
   MU &    33.3967749 &    0.0633803 &    0.0006398 &      -8e-07 &   -2.7102019 &    -4.06e-05 &     1.6e-06 \\
      &   (0.8468794) &  (0.5352262) &  (0.0039691) &     (4e-07) &  (0.8779943) &  (0.0002898) &     (5e-07) \\
      &               &              &              &             &              &              &             \\
   FB &    74.6863162 &   -0.1556568 &    0.0015774 &    -1.5e-06 &   -2.6450052 &    0.0001599 &     2.8e-06 \\
      &   (0.9171862) &  (1.1302096) &  (0.0064471) &     (9e-07) &  (0.7881093) &  (0.0009176) &     (1e-06) \\
      &               &              &              &             &              &              &             \\
 PCAR &    66.5653921 &   -0.0294768 &   -0.0044199 &    -6.3e-06 &   -2.6737082 &    -7.22e-05 &    1.15e-05 \\
      &   (0.6622394) &  (0.5652952) &  (0.0299058) &   (3.8e-06) &  (0.8936489) &  (0.0004809) &   (3.3e-06) \\
      &               &              &              &             &              &              &             \\
 AMZN &   317.2368614 &   -0.6234138 &    -0.005805 &   -3.45e-05 &   -2.6407034 &    0.0018582 &    6.83e-05 \\
      &  (14.3359568) &  (4.2419751) &  (0.2407367) &  (2.49e-05) &  (0.8677074) &  (0.0046468) &  (1.88e-05) \\
      &               &              &              &             &              &              &             \\
 EBAY &    54.1112839 &    0.0322441 &      6.2e-06 &    -1.5e-06 &   -2.7019206 &     4.68e-05 &       3e-06 \\
      &   (0.6804996) &  (0.4207827) &  (0.0079721) &     (9e-07) &  (0.9061468) &    (0.00035) &     (8e-07) \\
      &               &              &              &             &              &              &             \\
  SMH &    52.5152296 &    0.0492334 &   -0.0002052 &      -6e-07 &    -2.728325 &     -9.6e-06 &     1.1e-06 \\
      &   (1.0414812) &  (0.3983075) &  (0.0028926) &     (4e-07) &  (0.9110345) &  (0.0003551) &     (3e-07) \\
      &               &              &              &             &              &              &             \\
 INTC &    34.4930448 &     0.027989 &    0.0001221 &      -3e-07 &   -2.7783947 &     1.25e-05 &       8e-07 \\
      &   (1.1371134) &  (0.4241576) &  (0.0017873) &     (2e-07) &  (0.8585606) &  (0.0002294) &     (2e-07) \\
      &               &              &              &             &              &              &             \\
  VOD &    34.5712094 &   -0.0016934 &    -3.48e-05 &      -5e-07 &   -2.6613811 &     1.14e-05 &     1.2e-06 \\
      &   (1.2337536) &  (0.2765899) &   (0.003385) &     (4e-07) &  (0.9079183) &  (0.0001424) &     (4e-07) \\
      &               &              &              &             &              &              &             \\
 GOOG &   542.8337984 &   -0.0967683 &   -0.0168942 &   -4.72e-05 &   -2.6882949 &    0.0006758 &    9.34e-05 \\
      &   (6.1530034) &   (4.533289) &  (0.3071193) &   (3.9e-05) &  (0.8744376) &  (0.0055439) &  (2.64e-05) \\
      &               &              &              &             &              &              &             \\
 MSFT &    48.3945697 &    0.0601091 &    -7.33e-05 &      -4e-07 &   -2.7098915 &    -4.43e-05 &       8e-07 \\
      &   (0.7236829) &   (0.469177) &  (0.0020162) &     (2e-07) &  (0.9070437) &  (0.0002614) &     (2e-07) \\
      &               &              &              &             &              &              &             \\
\bottomrule
\end{tabular}
\end{table}


==> OFI_micro_latex-table <==
\begin{longtable}{lllllllllll}
\caption{Results for method ${OFI_{micro}}$}\\
\toprule
      Stock &           $a_0$ &         $a_1$ &          $a_2$ &        $a_3$ &          $a_4$ &    $adf-resid$ & $R^2_{OFI_{micro}}$ &     $\alpha$ &      $\beta$ & $R^2_{bench}$ \\
\midrule
\endhead
\midrule
\multicolumn{11}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
         MU &      33.3976715 &    -0.0061925 &      0.0001617 &       -8e-07 &     -0.0002785 &     -3.7419097 &           0.9053048 &    -4.06e-05 &      1.6e-06 &     0.6348812 \\
            &     (0.8449511) &   (0.1907172) &    (0.0022751) &      (3e-07) &    (0.0003134) &    (1.2216516) &         (0.0867001) &  (0.0002898) &      (5e-07) &   (0.1116312) \\
            &                 &               &                &              &                &                &                     &              &              &               \\
         FB &      74.6837965 &      0.053123 &       0.001143 &     -1.6e-06 &     -0.0004546 &       -3.36312 &           0.8879627 &    0.0001599 &      2.8e-06 &      0.646802 \\
            &     (0.9150394) &   (0.5698996) &    (0.0037318) &      (7e-07) &    (0.0005303) &    (0.9568442) &         (0.1077574) &  (0.0009176) &      (1e-06) &   (0.1213636) \\
            &                 &               &                &              &                &                &                     &              &              &               \\
       PCAR &      66.5654685 &    -0.0295009 &     -0.0021186 &     -6.5e-06 &      -0.001993 &     -3.4586142 &           0.8825702 &    -7.22e-05 &     1.15e-05 &     0.5943707 \\
            &     (0.6580494) &   (0.3106973) &    (0.0200821) &    (2.6e-06) &    (0.0022566) &    (1.0904161) &          (0.122286) &  (0.0004809) &    (3.3e-06) &   (0.0919139) \\
            &                 &               &                &              &                &                &                     &              &              &               \\
       AMZN &     317.2187288 &     0.2560108 &     -0.0121746 &     -3.8e-05 &     -0.0111251 &       -3.15502 &             0.81932 &    0.0018582 &     6.83e-05 &      0.497083 \\
            &    (14.3286014) &    (3.204889) &    (0.2088567) &   (1.94e-05) &    (0.0131955) &    (0.8397061) &         (0.1666376) &  (0.0046468) &   (1.88e-05) &   (0.1019693) \\
            &                 &               &                &              &                &                &                     &              &              &               \\
       EBAY &      54.1095513 &     0.0074091 &     -0.0003064 &     -1.5e-06 &     -0.0005658 &     -3.5466687 &           0.8985027 &     4.68e-05 &        3e-06 &     0.6237341 \\
            &     (0.6779297) &    (0.211954) &    (0.0048564) &      (6e-07) &    (0.0006356) &    (0.9679349) &         (0.0981883) &    (0.00035) &      (8e-07) &   (0.1201012) \\
            &                 &               &                &              &                &                &                     &              &              &               \\
        SMH &       52.513595 &     0.0264258 &      -6.32e-05 &       -6e-07 &     -0.0001945 &      -3.662269 &           0.9045901 &     -9.6e-06 &      1.1e-06 &     0.5366392 \\
            &      (1.042245) &    (0.213225) &    (0.0017799) &      (2e-07) &    (0.0002136) &    (1.0288569) &         (0.0835175) &  (0.0003551) &      (3e-07) &    (0.112495) \\
            &                 &               &                &              &                &                &                     &              &              &               \\
       INTC &      34.4921724 &     0.0070192 &      0.0001049 &       -4e-07 &       -0.00014 &     -3.8448383 &           0.9272422 &     1.25e-05 &        8e-07 &     0.6298803 \\
            &     (1.1357877) &    (0.144242) &    (0.0010034) &      (1e-07) &    (0.0001523) &    (1.2681683) &         (0.0654502) &  (0.0002294) &      (2e-07) &     (0.09795) \\
            &                 &               &                &              &                &                &                     &              &              &               \\
        VOD &      34.5696753 &     0.0076454 &       -7.8e-06 &       -5e-07 &     -0.0002337 &     -4.2250149 &            0.936199 &     1.14e-05 &      1.2e-06 &     0.5950157 \\
            &     (1.2324129) &   (0.1045205) &    (0.0017905) &      (2e-07) &    (0.0002649) &    (1.2164438) &         (0.0649528) &  (0.0001424) &      (4e-07) &   (0.1315352) \\
            &                 &               &                &              &                &                &                     &              &              &               \\
       GOOG &     542.8302421 &      0.328999 &     -0.0009426 &    -4.72e-05 &     -0.0145369 &     -3.1616662 &           0.8401094 &    0.0006758 &     9.34e-05 &     0.4950987 \\
            &     (6.1604382) &   (3.1658284) &     (0.235805) &    (2.7e-05) &     (0.017287) &    (0.9419513) &         (0.1517892) &  (0.0055439) &   (2.64e-05) &   (0.0956888) \\
            &                 &               &                &              &                &                &                     &              &              &               \\
       MSFT &      48.3980857 &    -0.0037844 &      -1.15e-05 &       -4e-07 &     -0.0001448 &     -3.7722162 &           0.9334051 &    -4.43e-05 &        8e-07 &     0.6882648 \\
            &     (0.7234343) &    (0.171465) &    (0.0008954) &      (1e-07) &    (0.0001574) &    (1.0471774) &         (0.0655859) &  (0.0002614) &      (2e-07) &   (0.0949067) \\
            &                 &               &                &              &                &                &                     &              &              &               \\
 Grand mean &  104.0390418378 &  0.0518920068 &  -0.0017076891 &  -8.2011e-06 &  -0.0024644319 &  -3.5487733524 &        0.8888303779 &  0.000274322 &  1.50546e-05 &  0.5966037586 \\
\end{longtable}

